Anteumbler: Non-Invasive Antenna Orientation Error Measurement for WiFi APs

The performance of WiFi-based localization systems is affected by the spatial accuracy of WiFi AP. Compared with the imprecision of AP location and antenna separation, the imprecision of AP's or antenna's orientation is more important in real scenarios, including AP rotation and antenna irregular tilt. In this paper, we propose Anteumbler that non-invasively, accurately and efficiently measures the orientation of each antenna in physical space. Based on the fact that the received power is maximized when a Tx-Rx antenna pair is perfectly aligned, we construct a spatial angle model that can obtain the antennas' orientations without prior knowledge. However, the sampling points of traversing the spatial angle need to cover the entire space. We use the orthogonality of antenna directivity and polarization and adopt an iterative algorithm to reduce the sampling points by hundreds of times, which greatly improves the efficiency. To achieve the required antenna orientation accuracy, we eliminate the influence of propagation distance using a dual plane intersection model and filter out ambient noise. Our real-world experiments with six antenna types, two antenna layouts and two antenna separations show that Anteumbler achieves median errors below 6 degree for both elevation and azimuth angles, and is robust to NLoS and dynamic environments. Last but not least, for the reverse localization system, we deploy Anteumbler over LocAP and reduce the antenna separation error by 10 mm, while for the user localization system, we deploy Anteumbler over SpotFi and reduce the user localization error by more than 1 m.

==> conclusion.tex <==
% \section{Conclusion} \label{sec:conclusion}
% This paper presents the design and implementation of \systemname, as far as we are aware, the first
% attempt to measure the orientation of each antenna of AP in physical space based on WiFi signals. \systemname \ makes two key technical contributions. First, it includes a spatial angle model, which can estimate the antenna orientation using only the CSI exposed by WiFi chips without extra requirements of the APs. Second, it contains an optimization model that fuses the orthogonality of electric field components, iterative loop algorithm and space geometry principles to achieve the accurate measurement of the AP's antennas orientations at the minute-level time cost, and eliminate the influence of propagation distance. Our real-world experiments with different antenna types, different antenna layouts and different environments show that \systemname \ achieves median errors below \SI{8}{^\circ} for both elevation and azimuth angles. 

==> related_work.tex <==
% \section{Related Work} \label{sec:related}
% We briefly review the related work with \oursystem \ from three aspects.

% \textbf{WiFi localization and tracking.}
% Due to its ubiquitous deployment, WiFi has been extensively studied for indoor localization and tracking in the past two decades. Some of the initial work is based on RSSI~\cite{832252,10.1145/1859995.1860016,zhu2013rssi}, but these algorithms usually require a lot of fingerprint to achieve decimeter-level localization accuracy. Therefore, most recent works focus on localization algorithms based on fine-grained CSI~\cite{10.1145/2639108.2639139,10.1145/2639108.2639142,10.1145/3210240.3210347,10.5555/2930611.2930623,ArrayTrack,spotfi,10.1145/2789168.2790125}, and their commonly used localization ideas include AoA-based~\cite{ArrayTrack,spotfi}, ~\emph{time of flight} (ToF)-based~\cite{10.1145/2462456.2464463,10.5555/2930611.2930623,kotaru2017position}, and fusion of AoA and ToF~\cite{10.1145/3372224.3380894,mD-Track}. Many systems can achieve decimeter-level localization accuracy using commercial WiFi. However, these WiFi-based localization systems do not take into account the effects of APs' or antennas' orientation errors, they assume that the APs' and antennas' orientations are precisely known and parallel to ensure accurate antenna separation for estimating user location. Compared with the above works, we quantitatively analyze the effect of APs' or antennas' orientation errors on localization accuracy, and construct an antenna orientation estimation method that can accurately estimate the orientation of each antenna on the AP. The accuracy of the localization system is guaranteed by correction the antenna orientation.


% % \textbf{Reverse localization of WiFi AP.}
% % WiFi-based localization systems assume accurate knowledge of AP locations, orientations and antenna geometry, but in the real world, these AP attribute information is often unknown or inaccurate, making WiFi localization difficult to deploy~\cite{locap2020}. Reverse localization is designed to solve this problem by obtaining AP attribute information autonomously. There are some works on the reverse localization of WiFi AP~\cite{10.1145/1859995.1860016,8928047,locap2020,MapFi2021}. LocAP~\cite{locap2020} systematically analyzes the influence of spatial attributes such as AP's location, orientation and antenna separation on the localization accuracy, and based on the SLAM robot, it realizes autonomous mapping of these spatial attributes of APs in unknown physical maps. MapFi~\cite{MapFi2021} proposes an estimation method of ~\emph{angle difference of arrival} (ADoA) for many heterogeneous WiFi APs and various antenna layouts. It only needs to know the locations of three APs in advance, so that APs with different antenna layouts can locate each other without additional equipment. However, they can only measure different orientations of APs in the horizontal plane, and they all assume that all antennas on the AP are parallel. In contrast to these works, \oursystem \ estimates the orientation of each antenna, which in turn ensures the accuracy of WiFi AP reverse localization.

% % \textbf{Estimation of antenna orientation.}
% % Traditionally, there are some methods to estimate the elevation and azimuth angles of the antenna. For example, the antenna orientation is manually measured or calibrated using a compass~\cite{compass} and inclinometer~\cite{inclinometer}. There are also integrated systems on the antenna that can automatically measure the antenna orientation~\cite{cpi-2.4aebp}. But these are labor intensive or require the antenna to be equipped with sensors. To the best of our knowledge, \oursystem \ is the first attempt to estimate antenna elevation and azimuth angles based on commercial WiFi signals.



